VRMN-bD: A Multi-modal Natural Behavior Dataset of Immersive Human Fear Responses in VR Stand-up Interactive Games

Understanding and recognizing emotions are important and challenging issues in the metaverse era. Understanding, identifying, and predicting fear, which is one of the fundamental human emotions, in virtual reality (VR) environments plays an essential role in immersive game development, scene development, and next-generation virtual human-computer interaction applications. In this article, we used VR horror games as a medium to analyze fear emotions by collecting multi-modal data (posture, audio, and physiological signals) from 23 players. We used an LSTM-based model to predict fear with accuracies of 65.31% and 90.47% under 6-level classification (no fear and five different levels of fear) and 2-level classification (no fear and fear), respectively. We constructed a multi-modal natural behavior dataset of immersive human fear responses (VRMN-bD) and compared it with existing relevant advanced datasets. The results show that our dataset has fewer limitations in terms of collection method, data scale and audience scope. We are unique and advanced in targeting multi-modal datasets of fear and behavior in VR stand-up interactive environments. Moreover, we discussed the implications of this work for communities and applications. The dataset and pre-trained model are available at https://github.com/KindOPSTAR/VRMN-bD.

==> Experimental-procedure.tex <==
\begin{document}

\begin{table*}[!ht]
\centering
\caption{Experimental procedure. The reading order starts from the top left corner and goes from top to bottom and left to right in stage and period order. Stage is included in the period.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\begin{tabular}[c]{@{}c@{}}Period\\ /Stage\end{tabular} &
  Preparation &
  \begin{tabular}[c]{@{}c@{}} Game 1\\ (Richie's Plank Experience)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} Game 2\\ (Phasmophobia)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} Game 3\\ (Emily wants to play)\end{tabular} &
  Post-experimental stage \\ \hline
1 &
  \begin{tabular}[c]{@{}c@{}}Start of \\ experimental procedure\end{tabular}  &
  \begin{tabular}[c]{@{}c@{}}Configuration of the game*.\\ Learn about basic operation methods \\ and tasks that need to be completed.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Configure the game*, including \\ selecting a specific game difficulty, \\ a specific game map, \\ and pre-equipping props.\\ Learn about basic operation methods \\ and tasks$^{\alpha}$ that need to be completed.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Configure the game*, including \\ selecting a specific game difficulty, \\ a specific game map, \\ and pre-equipping props.\\ Learn about basic operation methods \\ and tasks$^{\alpha}$ that need to be completed.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Completion of \\ the post-test Panas-X scale\end{tabular} \\
2 &
  \begin{tabular}[c]{@{}c@{}}Check in: Fill in the informed \\ consent, questionary \\ and pre-test Panas-X scale\end{tabular} &
  Start of the VR experience for Game 1 &
  Start of the VR experience for Game 2 &
  Start of the VR experience for Game 3 &
  \begin{tabular}[c]{@{}c@{}}Remove the device used to \\ record physiological signals\\ and voice recording\end{tabular} \\
3 &
  \begin{tabular}[c]{@{}c@{}}Wearing devices for \\ detecting physiological signals \\ (heart and breathing rate).\\Wearing a wireless microphone\\ on the lapel.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Part 1 (step-by-step \\ and task-based):\\ (1) Walking at height;\\ (2) Fright from spiders;\\ (3) High falling.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}The player explores the room \\ in complete darkness, \\ illuminated only by a white flashlight \\ and a purple flashlight.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Players explore a dimly lit room \\ with a jumble of objects \\ containing broken mirrors, \\ creepy dolls, \\ suddenly disappearing humanoid shadows\\  and notes with hints of horror.\end{tabular} &
  Payment to participants* \\
4 &
  \begin{tabular}[c]{@{}c@{}}Non-horror VR Tutorial for Beginners, \\ this will take about 5 minutes \\ and participants will learn \\ how to use the VR device \\ in this step by step process.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Active triggering of organs \\ without warning (task-based). \\ The game screen changes \\ to a cold tone after triggering.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}The game process is accompanied \\ by random thunder, \\ walking sounds, sounds of close/open doors, \\ fluorescent handprints, and flashing flashlights.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}The game process is accompanied \\ by thunder, sounds of close/open doors, \\ random lights on and off with sounds.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}End of experience for \\ whole experimental procedure,\\ and\\  participants can go to \\ the waiting room to \\ wait for other participants or\\  free to leave.\end{tabular} \\
5 &
  Move to Game 1 &
  \begin{tabular}[c]{@{}c@{}}Part 2 (step-by-step):\\ (1) The spider meets the face;\\ (2) Walking at height (task-based);\\ (3)  High falling;\\ (4) Dentist in a dark environment;\\ (5)  Car head-on crash.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Around the 15th minute after the game starts, \\ the player enters a near-death state, \\ accompanied by high-frequency \\ flashing flashlight lights, \\ footsteps, and possible ghostly figures.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}About 5 minutes after the game starts, \\ the player will hear a eerie girl laugh \\ and a standing eerie girl doll \\ will appear next to the player \\ (previously in a sitting position).\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Use 75\% ethyl alcohol to \\ clean and disinfect \\ the relevant equipment*.\end{tabular} \\
6 &
   &
  End of  VR experience for Game 1 &
  \begin{tabular}[c]{@{}c@{}}The flashlight dropped, \\ and a pair of scary hands \\ blinded the player's vision.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Once the player line of \\ sight away from the doll, \\ then there will be a horrible face \\ of jump scare$^{\beta}$.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Move to the next round \\ of the experimental process \\ and repeat this procedure \\ until the data collection part \\ is completed.\end{tabular} \\
7 &
  \multicolumn{1}{l}{} &
  \begin{tabular}[c]{@{}c@{}}Game 1 based questionnaires and interviews:\\ (1) Completion of chapter questionnaires;\\ (2) Subjective report interviews \\ based on recent game experiences.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Players enter the soul state \\ and can see their own "corpse," \\ and the game screen becomes pale.\end{tabular} &
  End of  VR experience for Game 3 &
  \multicolumn{1}{l}{} \\
8 &
  \multicolumn{1}{l}{} &
  \begin{tabular}[c]{@{}c@{}}End of the experimental procedure\\  for Game 1, and move to Game 2\end{tabular} &
  End of  VR experience for Game 2 &
  \begin{tabular}[c]{@{}c@{}}Game 3 based questionnaires and interviews:\\ (1) Completion of chapter questionnaires;\\ (2) Subjective report interviews \\ based on recent game experiences.\end{tabular} &
  \multicolumn{1}{l}{} \\
9 &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \begin{tabular}[c]{@{}c@{}}Game 2 based questionnaires and interviews:\\ (1) Completion of chapter questionnaires;\\ (2) Subjective report interviews \\ based on recent game experiences.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}End of the experimental procedure\\  for Game 3, \\ and move to \\ post-experimental stage\end{tabular} &
  \multicolumn{1}{l}{} \\
10 &
   &
   &
  \begin{tabular}[c]{@{}c@{}}End of the experimental procedure\\  for Game 2, and move to Game 3\end{tabular} &
   &
   \\ \bottomrule
\multicolumn{6}{l}{* host tasks} \\
\multicolumn{6}{l}{$^{\alpha}$ false tasks} \\
\multicolumn{6}{l}{$^{\beta}$ The real gameplay that is not informed to the player, if triggered, will have multiple rounds of repetition until failure.}
\end{tabular}%
}
\label{tab:experimental procedure}
\end{table*}


\end{document}


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

